Proceedings of the third French-Ukrainian workshop on the instrumentation developments for HEP

The reports collected in these proceedings have been presented in the third French-Ukrainian workshop on the instrumentation developments for high-energy physics held at LAL, Orsay on October 15-16. The workshop was conducted in the scope of the IDEATE International Associated Laboratory (LIA). Joint developments between French and Ukrainian laboratories and universities as well as new proposals have been discussed. The main topics of the papers presented in the Proceedings are developments for accelerator and beam monitoring, detector developments, joint developments for large-scale high-energy and astroparticle physics projects, medical applications.

==> first/picture.tex <==
\pagestyle{plain}
\addcontentsline{toc}{section}{\textbf{Picture}}
\normalsize

\usepackage{epsfig}

\vskip 1cm

% \noindent

\begin{figure} [htb]
\begin{center}
\mbox{\epsfig{figure=first/participants.eps,height=11.0cm}}
% \caption{}
\end{center}
\end{figure}

Participants of the workshop, LAL, Orsay, 16 October 2015

\vskip 2cm

URL: http://french-ukrainian-workshop-2015.lal.in2p3.fr/

\vskip 5.5cm

 Edited by F.A. Danevich

 23 December 2015

